$\Lambda\rm{K}$ femtoscopy in Pb-Pb collisions at $\sqrt{s_{\rm{NN}}}$ = 2.76 TeV

The first measurements of the scattering parameters of $\Lambda$K pairs in all three charge combinations ($\Lambda$K$^{+}$, $\Lambda$K$^{-}$, and $\Lambda\mathrm{K^{0}_{S}}$) are presented. The results are achieved through a femtoscopic analysis of $\Lambda$K correlations in Pb-Pb collisions at $\sqrt{s_{\mathrm{NN}}}$ = 2.76 TeV recorded by ALICE at the LHC. The femtoscopic correlations result from strong final-state interactions, and are fit with a parametrization allowing for both the characterization of the pair emission source and the measurement of the scattering parameters for the particle pairs. Extensive studies with the THERMINATOR 2 event generator provide a good description of the non-femtoscopic background, which results mainly from collective effects, with unprecedented precision. Furthermore, together with HIJING simulations, this model is used to account for contributions from residual correlations induced by feed-down from particle decays. The extracted scattering parameters indicate that the strong force is repulsive in the $\Lambda\rm{K}^{+}$ interaction and attractive in the $\Lambda\rm{K}^{-}$ interaction. The data hint that the and $\Lambda\rm{K}^{0}_{S}$ interaction is attractive, however the uncertainty of the result does not permit such a decisive conclusion. The results suggest an effect arising either from different quark-antiquark interactions between the pairs ($\rm s\overline{s}$ in $\Lambda$K$^{+}$ and $\rm u\overline{u}$ in $\Lambda$K$^{-}$) or from different net strangeness for each system (S = 0 for $\Lambda$K$^{+}$, and S = $-2$ for $\Lambda$K$^{-}$). Finally, the $\Lambda$K systems exhibit source radii larger than expected from extrapolation from identical particle femtoscopic studies. This effect is interpreted as resulting from the separation in space-time of the single-particle $\Lambda$ and K source distributions.

==> ResultsTable/TableHelperTriple.tex <==
\newarray\ArrLamKchP
\readarray{ArrLamKchP}{
                       1.14 & 0.29 & 0.18 & 
                       6.02 & 0.82 & 0.65 & 
                       0.82 & 0.18 & 0.16 & 
                       4.50 & 0.51 & 0.45 & 
                       0.90 & 0.22 & 0.19 & 
                       3.61 & 0.44 & 0.30 & 
                       $-$0.60 & 0.12 & 0.11 & 
                       0.51 & 0.15 & 0.12 & 
                       0.83 & 0.47 & 1.23}

\newarray\ArrALamKchM
\readarray{ArrALamKchM}{
                       1.14 & 0.29 & 0.18 & 
                       6.02 & 0.82 & 0.65 & 
                       0.82 & 0.18 & 0.16 & 
                       4.50 & 0.51 & 0.45 & 
                       0.90 & 0.22 & 0.19 & 
                       3.61 & 0.44 & 0.30 & 
                       $-$0.60 & 0.12 & 0.11 & 
                       0.51 & 0.15 & 0.12 & 
                       0.83 & 0.47 & 1.23}

\newarray\ArrLamKchM
\readarray{ArrLamKchM}{
                       1.14 & 0.29 & 0.18 & 
                       6.02 & 0.82 & 0.65 & 
                       0.82 & 0.18 & 0.16 & 
                       4.50 & 0.51 & 0.45 & 
                       0.90 & 0.22 & 0.19 & 
                       3.61 & 0.44 & 0.30 & 
                       0.27 & 0.12 & 0.07 & 
                       0.40 & 0.11 & 0.07 & 
                       $-$5.23 & 2.13 & 4.80}

\newarray\ArrALamKchP
\readarray{ArrALamKchP}{
                       1.14 & 0.29 & 0.18 & 
                       6.02 & 0.82 & 0.65 & 
                       0.82 & 0.18 & 0.16 & 
                       4.50 & 0.51 & 0.45 & 
                       0.90 & 0.22 & 0.19 & 
                       3.61 & 0.44 & 0.30 & 
                       0.27 & 0.12 & 0.07 & 
                       0.40 & 0.11 & 0.07 & 
                       $-$5.23 & 2.13 & 4.80}

\newarray\ArrLamKs
\readarray{ArrLamKs}{
                       1.14 & 0.29 & 0.18 & 
                       6.02 & 0.82 & 0.65 & 
                       0.82 & 0.18 & 0.16 & 
                       4.50 & 0.51 & 0.45 & 
                       0.90 & 0.22 & 0.19 & 
                       3.61 & 0.44 & 0.30 & 
                       0.10 & 0.13 & 0.07 & 
                       0.58 & 0.15 & 0.13 & 
                       $-$1.85 & 1.71 & 2.77}

\newarray\ArrALamKs
\readarray{ArrALamKs}{
                       1.14 & 0.29 & 0.18 & 
                       6.02 & 0.82 & 0.65 & 
                       0.82 & 0.18 & 0.16 & 
                       4.50 & 0.51 & 0.45 & 
                       0.90 & 0.22 & 0.19 & 
                       3.61 & 0.44 & 0.30 & 
                       0.10 & 0.13 & 0.07 & 
                       0.58 & 0.15 & 0.13 & 
                       $-$1.85 & 1.71 & 2.77}


